Emotion Flip Reasoning in Multiparty Conversations

In a conversational dialogue, speakers may have different emotional states and their dynamics play an important role in understanding dialogue's emotional discourse. However, simply detecting emotions is not sufficient to entirely comprehend the speaker-specific changes in emotion that occur during a conversation. To understand the emotional dynamics of speakers in an efficient manner, it is imperative to identify the rationale or instigator behind any changes or flips in emotion expressed by the speaker. In this paper, we explore the task called Instigator based Emotion Flip Reasoning (EFR), which aims to identify the instigator behind a speaker's emotion flip within a conversation. For example, an emotion flip from joy to anger could be caused by an instigator like threat. To facilitate this task, we present MELD-I, a dataset that includes ground-truth EFR instigator labels, which are in line with emotional psychology. To evaluate the dataset, we propose a novel neural architecture called TGIF, which leverages Transformer encoders and stacked GRUs to capture the dialogue context, speaker dynamics, and emotion sequence in a conversation. Our evaluation demonstrates state-of-the-art performance (+4-12% increase in F1-score) against five baselines used for the task. Further, we establish the generalizability of TGIF on an unseen dataset in a zero-shot setting. Additionally, we provide a detailed analysis of the competing models, highlighting the advantages and limitations of our neural architecture.

==> 2_Problem_Definition.tex <==
The EFR task can be formally defined as follows:
Given a sequence of $n$ tuples of the form $\langle u_i, s_j, e_k \rangle$ in a multiparty conversation, where $s_j \in S$ is a speaker from a predefined speaker set $S$, $e_k \in E$ is a set of emotion labels, and $u_i \in D$ is an utterance of the dialogue $D$, we associate instigator label(s) with an utterance $u_l$ if it causes a flip/change in emotion of a speaker $s_m\in S$ in her consecutive utterances in the conversation. We define the objective in the following three steps.  

\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
    \item First, we identify all utterances $u_i$ in a dialogue which experience an emotion flip of some speaker $s_j$ -- when the emotion for the utterance %$u_j^{s_i}$ 
    is different from the emotion associated with the last utterance of speaker $s_j$. We call $u_i$ as the target utterance. 
    
    \item Second, for each emotion flip utterance $u_i$, we mark a set of previous utterances $u_k \in \{u_1, u_2, \cdots, u_i\}$  which are responsible for the emotion flip at $u_i$. Note that the current utterance $u_i$ can also be responsible for the emotion flip. 
    
    \item Finally, we associate psychologically motivated instigator labels (c.f. Section \ref{sec:dataset}) to each $u_k$ for a target utterance $u_i$.  
\end{itemize}

Figure \ref{fig:data_example2} illustrates an example of emotion flip with corresponding instigators. It shows a multiparty scenario where three speakers are engaged in a conversation. There are two emotion flips -- $\langle u_1, Ross, fear\rangle$ $\rightarrow$ $\langle u_3, Ross, joy\rangle$  and $\langle u_3, Ross, joy\rangle$ $\rightarrow$ $\langle u_5, Ross, anger\rangle$. The first flip occurs due to two trigger utterances, $u_2$  and $u_3$, with different set of instigator labels (\textit{Nervousness} and \textit{Adoration}). On the other hand, the trigger for the second flip is a single utterance ($u_4$), and the corresponding instigator labels are \textit{Annoyance} and \textit{Challenge}. This example highlights the case when more than one trigger utterance can cause an emotion flip.

==> fig_data_example2.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{example1new.pdf}
    \caption{Example of an emotion flip with self-trigger. Monica's emotion flipped from \textit{Neutral} ($u_1$) to \textit{Sadness} ($u_3$) due to one trigger utterance ($u_3$ itself) caused by the instigators \textit{nostalgia} and \textit{loss}. The other speaker's emotion then flipped from \textit{Joy} ($u_2$) to \textit{Surprise} ($u_4$) due to a single trigger utterance ($u_3$ again) caused by the instigators \textit{nostalgia}, \textit{loss} and \textit{shock}.}
    \label{fig:data_example1}
\end{figure*}

==> tab_coarse-grained-error.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|p{15em}|c|c|c|p{10em}|p{10em}|}
\hline
\multirow{3}{*}{} & \multirow{3}{*}{\textbf{Speaker}} & \multirow{3}{*}{\textbf{Utterance}} & \multirow{3}{*}{\textbf{Emotion}} & \multirow{3}{*}{\textbf{Tr}} & \multicolumn{3}{c|}{\textbf{Instigators}} \\ \cline{6-8}
 & & & & & \multirow{2}{*}{\textbf{Gold}} & \multicolumn{2}{c|}{\textbf{Prediction}} \\ \cline{7-8}
 & & & & & & \textbf{\name} &  \textbf{BERT}  \\ \hline
\hline
$u_1$ & Ross & Okay, go left. Left! Left! & surprise & 0 & - & - & - \\ \hline
$u_2$ & Rachel & Okay, y'know what? There is no more left, left! & anger & 1 & \multirow{2}{5em}{annoyance, nervousness} & {annoyance, nervousness, {\color[HTML]{FE0000}awkwardness, loss, others}} & nervousness, {\color[HTML]{FE0000}awkwardness, benefit, cheer, others} \\ \hline
$u_3$ & Ross & Oh okay, lift it straight up over your head! & anger & 0 & - & - & -  \\ \hline
\end{tabular}%
}
\caption{Coarse-grained analysis: Actual and predicted instigator labels for an EFR instance. \name\ predicts both the correct instigator labels for the trigger utterance, $u_2$. It wrongly predicts three instigators. In contrast, BERT only predicts one correct label and four false positives.}
\label{tab:error14}
\end{table*}


==> tab_dataset_creation2.tex <==
\begin{table*}[h!]

\centering

\subfloat[An example dialogue from MELD]{
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l}
    \cline{1-4} 
     & \bf Speaker & \bf Utterance & \bf Em & \\ \cline{1-4}
     $u_1$ & Monica & You wanna hear something that sucks? & Neu & \\ \cline{1-4}
     $u_2$ & Chandler & Do I ever? & Joy \\ \cline{1-4}
     $u_3$ & Monica & Chris says they’re closing down the bar. & Sad & \cellcolor{LightCyan} Emotion flip - 1 \\ \cline{1-4}
     $u_4$ & Chandler & No way! & Sur & \cellcolor{LightCyan} Emotion flip - 2 \\ \cline{1-4}
 \end{tabular}
 }}
\\
\subfloat[Instance - 1]{
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
    \hline 
     & \bf Speaker & \bf Utterance & \bf Em \\ \hline
     $u_1$ & Monica & You wanna hear something that sucks? & Neu\\ \hline
     $u_2$ & Chandler & Do I ever? & Joy \\ \hline
     \rowcolor{LightCyan} $u_3$ & Monica & Chris says they’re closing down the bar. & Sad \\ \hline
\end{tabular}}
}
\hspace{1em} 
\subfloat[MELD-I Annotation: Trigger/Instigator]{
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|p{5em}|}
    \hline 
     & \bf Speaker & \bf Utterance & \bf Em & \bf Trigger & \bf Instigator \\ \hline
     $u_1$ & Monica & You wanna hear something that sucks? & Neu & No & - \\ \hline
     $u_2$ & Chandler & Do I ever? & Joy & No & - \\ \hline
     $u_3$ & Monica & Chris says they’re closing down the bar. & Sad & Yes & Nostalgia, Loss \\ \hline
\end{tabular}}
}
\\
\subfloat[Instance - 2]{
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
    \hline 
     & \bf Speaker & \bf Utterance & \bf Em \\ \hline
     $u_1$ & Monica & You wanna hear something that sucks? & Neu\\ \hline
     $u_2$ & Chandler & Do I ever? & Joy \\ \hline
     $u_3$ & Monica & Chris says they’re closing down the bar. & Sad \\ \hline
     \rowcolor{LightCyan} $u_4$ & Chandler & No way ! & Sur \\ \hline
\end{tabular}
}}
\hspace{1em} 
\subfloat[MELD-I Annotation: Trigger/Instigator]{
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|p{5em}|}
    \hline 
     & \bf Speaker & \bf Utterance & \bf Em & \bf Trigger & \bf Instigator \\ \hline
     $u_1$ & Monica & You wanna hear something that sucks? & Neu & No & - \\ \hline
     $u_2$ & Chandler & Do I ever? & Joy & No & -\\ \hline
     $u_3$ & Monica & Chris says they’re closing down the bar. & Sad & Yes & Nostalgia, Loss, Shock \\ \hline
     \rowcolor{LightCyan} $u_4$ & Chandler & No way ! & Sur & No & - \\ \hline
\end{tabular}
}}
\caption{Dataset development for an instance shown in Figure \ref{fig:data_example1}. \textbf{a)} \textit{Original dialogue from MELD}; \textbf{b,d)} \textit{Two instances corresponding to the two emotion flips in a.} \textbf{c,e)} \textit{Trigger and instigator annotations for both instances.}}
\label{tab:data_creation1}
\end{table*}

==> tab_hyperparameters.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{4}{*}{\textbf{Global}} & \textbf{Batch Size} & \multicolumn{2}{c|}{64} \\ \cline{2-4} 
 & \textbf{Learning Rate} & \multicolumn{2}{c|}{1e-3} \\ \cline{2-4} 
 & \textbf{\# Epochs} & \multicolumn{2}{c|}{100} \\ \cline{2-4} 
 & \textbf{Fully connected Module} & \multicolumn{2}{c|}{1634 $\rightarrow$ 800 $\rightarrow$ 400 $\rightarrow$ 100 $\rightarrow$ 27/14} \\ \hline
\multirow{6}{*}{\textbf{Transformer Encoder}} & \textbf{} & \textbf{GUS} & \textbf{GSS} \\ \cline{2-4} 
 & \textbf{Input Size} & 768 & 8 \\ \cline{2-4} 
 & \textbf{\# Layers} & 4 & 4 \\ \cline{2-4} 
 & \textbf{\# Attention Heads} & 4 & 4 \\ \cline{2-4} 
 & \textbf{Feedforward dimension} & 2048 & 2048 \\ \cline{2-4} 
 & \textbf{Dropout} & 0.2 & 0.2 \\ \hline
\multirow{5}{*}{\textbf{GRU}} & \textbf{} & \textbf{GES} & \textbf{SESS} \\ \cline{2-4} 
 & \textbf{Input Size} & 7 & 7 \\ \cline{2-4} 
 & \textbf{\# Layers} & 2 & 2 \\ \cline{2-4} 
 & \textbf{Hidden Size} & 10 & 10 \\ \cline{2-4} 
 & \textbf{Output Size} & 7 & 10 \\ \hline
\end{tabular}
}
\caption{Hyperparameters used in our model to obtain the reported results.}
\label{tab:hyperparams}
\end{table}

==> tab_results_14_250.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c||c|}
\hline
\textbf{Model} & \textbf{AGHMN} & \textbf{TL-ERC} & \textbf{DGCN} & \textbf{DialogXL} & \textbf{TGIF} \\ \hline
\textbf{Weighted F1} & 12.8 & 21.7 & 28.3 & 13.6 & \textbf{37.5} \\ \hline
\end{tabular}%
}
\caption{Comparative results on count based level-1 instigators. \hl{Need precision and recall here as well. Try merging this table with 5.}}
\label{tab:results_classes14_250}
\end{table}
